Practical Batch Bayesian Optimization for Less Expensive Functions

Bayesian optimization (BO) and its batch extensions are successful for optimizing expensive black-box functions. However, these traditional BO approaches are not yet ideal for optimizing less expensive functions when the computational cost of BO can dominate the cost of evaluating the blackbox function. Examples of these less expensive functions are cheap machine learning models, inexpensive physical experiment through simulators, and acquisition function optimization in Bayesian optimization. In this paper, we consider a batch BO setting for situations where function evaluations are less expensive. Our model is based on a new exploration strategy using geometric distance that provides an alternative way for exploration, selecting a point far from the observed locations. Using that intuition, we propose to use Sobol sequence to guide exploration that will get rid of running multiple global optimization steps as used in previous works. Based on the proposed distance exploration, we present an efficient batch BO approach. We demonstrate that our approach outperforms other baselines and global optimization methods when the function evaluations are less expensive.

==> experiment_v6.tex <==
We aim to illustrate that our models can reasonably estimate the
unknown number of discriminative clusters and improve the clustering
performance.

\paragraph{Experimental setup.}

All experiments are running in the same  Windows machine Core i7,
16GB of RAM. The implementation of the proposed model and the baselines
are in Matlab. Throughout the experiments, the prior distribution
for $\boldsymbol{\eta}_{k}$ is set as $p\left(\boldsymbol{\eta}_{k}\mid\mu_{0},\Sigma_{0}\right)\sim\mathcal{N}\left(0,\idenmat\right)$.
We use symmetric Dirichlet with parameter $0.01$.\textit{\emph{ We
set the hyperparameters as $\alpha,\gamma\sim\gammapdf(1,1)$}},
then we resample them in each iteration (for robustness) following
the approaches presented in \cite{Escobar_West_95bayesian,Teh_etal_06hierarchical}.

To have a good initialization for each discriminative models, in the
first 10 iterations of the collapsed Gibbs sampler, we run our proposed
models without using discriminative property. We call our discriminative
DPM with SVM (DDPM-S) and with LR (DDPM-L). Similarly, DIH-S and DIH-L\emph{
}refer to the two variants of discriminative state iHMM. For evaluation,
the clustering scores are measured using 10 independent runs, for
each run we record the results from the last 5 Gibbs samples to reduce
the sensitivity of MCMC.
\begin{figure}
\begin{centering}
\includegraphics[width=0.95\columnwidth]{figs/experiment_synthetic/DPM_Iter_300_caption}
\par\end{centering}
\begin{centering}
\includegraphics[width=0.95\columnwidth]{figs/experiment_synthetic/DDPM-S_Iter_30_caption}
\par\end{centering}
\caption{Clustering on the linearly chained Gaussians. We note that if we exhaustively
tune the Gaussian covariance hyperparameter controlling the horizontal
shape, DPM will estimate correctly. In contrast, by utilizing the
discriminative property, DDPM can learn the pattern successfully without
tuning the covariance. \label{fig:Synthetic_Data-2}}

\vspace{-2pt}
\end{figure}

\begin{table*}
\begin{centering}
\begin{tabular}{|l|>{\centering}p{20pt}|c|c|c|>{\centering}p{37pt}|c|c|c|c|}
\hline 
 & Score & Kmeans & GMM & AP & DPmeans & DPM & MMGM & DDPM-L & DDPM-S\tabularnewline
\hline 
\hline 
\multirow{3}{*}{\begin{turn}{90}
NUS
\end{turn}} & K & {\small{}10-25} & {\small{}10-25} & 18 & 17 & 19 & 15 & 15 & 17\tabularnewline
\cline{2-10} 
 & NMI & .18(.01) & .19(.01) & .166 & .161 & .191(.006) & .184(.007) & \textbf{\emph{.197(.012)}} & \textbf{.199(.005)}\tabularnewline
\cline{2-2} 
 & F1 & .16(.01) & .16(.01) & .145 & .166 & .172(.003) & \textbf{\emph{.177(.01)}} & .175(.011) & \textbf{.180(.007)}\tabularnewline
\hline 
\multirow{3}{*}{\begin{turn}{90}
Scenes
\end{turn}} & K & {\small{}10-25} & {\small{}10-25} & 18 & 17 & 12 & 10 & 11 & 12\tabularnewline
\cline{2-10} 
 & NMI & .16(.02) & .17(.02) & .154 & .155 & .208(.006) & .186(.008) & \textbf{\emph{.218(.01)}} & \textbf{.217(.02)}\tabularnewline
\cline{2-2} 
 & F1 & .13(.01) & .12(.01) & .124 & .148 & .172(.006) & .171(.009) & \textbf{.178(.01)} & \textbf{\emph{.176(.02)}}\tabularnewline
\hline 
\multirow{3}{*}{\begin{turn}{90}
Mnist
\end{turn}} & K & {\small{}10-25} & {\small{}10-25} & 18 & 17 & {\small{}20} & 18 & 16 & 14\tabularnewline
\cline{2-10} 
 & NMI & 0.56(.02) & .52(.03) & .471 & .518 & \textbf{\emph{.603(.02)}} & .583(.02) & \textbf{.617(.02)} & .597(.04)\tabularnewline
\cline{2-2} 
 & F1 & .40(.03) & .38(.02) & .327  & .379 & .395(.01) & .420(.02) & \textbf{\emph{.481(.02)}} & \textbf{.457(.03)}\tabularnewline
\hline 
\end{tabular}
\par\end{centering}
\caption{Image clustering comparison. The best and second best scores are
in \textbf{bold} and \textbf{\emph{italic}}. \label{tab:NUS_ImageClustering-1}}
\end{table*}


\subsection{DDPM for Data Clustering}

We conduct experiments for DDPM on synthetic linear-shape Gaussian
2D data and image clustering task where the data include a collection
of i.i.d. observations.

\subsubsection{Synthetic experiment}

We offer a simple illustration to understand the advantage of discriminative
clustering (against the standard clustering methods) in Fig. \ref{fig:Synthetic_Data-2}.
DDPM-S and DDPM-L  recover correctly $K=2$ clusters while DPM cannot
recover the true clusters. Both DDPM and DPM use Gaussian likelihood
to encourage the similarity of data points within a cluster. In addition,
the discriminative hyperplane $\boldsymbol{\eta}_{k}$ in DDPM helps
to separate data points in the $k$-th cluster to be away from other
clusters. This property makes the algorithm converge to a fewer
number of clusters while gaining better clustering performance. We
note that if we exhaustively tune the covariance of the Gaussian
distribution, DPM might estimate these clusters correctly; whereas
our model achieves this with minimum effort.

\subsubsection{Image clustering}

We evaluate DDPM on image clustering using NUS Wide (K=13, N=3411,
D=500), Fifteen Scenes (K=15, N=2245, D=128) and MNIST (K=10, N=1000,
D=784) datasets where K is the number of true cluster, N is the number
of data points and D is the feature dimension. We use SIFT histogram
as a feature which is assumed to follow Multinomial distribution \cite{nguyen_phung_nguyen_venkatesh_bui_icml14,Nguyen_2015Large}. 

We compare our models with the  existing methods:

\emph{DPM} \cite{Antoniak_74mixtures}: we use the same configuration
with our proposed model. 

\emph{MMGM} \cite{Chen_2014Robust}: Since Gaussian-Wishart for high
dimensional count data of SIFT vectors is not effective, we use Multinomial-Dirichlet
likelihood.

\emph{DPmeans} \cite{Kulis_Jordan_12Revisiting}: We follow \cite{Kulis_Jordan_12Revisiting}
method to select $\lambda$ using farthest-first heuristic where the
expected number of cluster is set to $17$ to estimate $\lambda$.
This yields $\lambda=5690$.

\emph{K-means}\textbf{,} \emph{GMM} and \emph{AP} \cite{Frey_Dueck_07clustering}:
We use Matlab built-in function with Euclidean distance. As K-means
and GMM require the number of clusters provided in advance, we vary
the number of clusters from 10 to 25, then report the mean and standard
deviation.

Table \ref{tab:NUS_ImageClustering-1} shows the clustering results.
DP-means \cite{Kulis_Jordan_12Revisiting} achieves much lower scores
than DPM and DDPM in clustering quality. DP-means uses small-variance
asymptotic analysis and uses the mean of the data to represent a
center. This trade-off assumption makes the DP-means deterministic
as traditional k-means, hence run faster, but it degrades the clustering
performance. GMM and Kmeans require the number of clusters provided
in advance. To have a fair comparison with other BNP approaches which
can identify the suitable number of clusters, we vary the number of
clusters used in GMM and Kmeans, then report the mean and standard
deviation. Our discriminative models consistently achieve the best
clustering quality as they outperform the other baselines in all NMI
and F1-score. Among our two discriminative variants, DDPM-S with the
hinge loss performs slightly better than DDPM-L with the logistic
loss. 

Our model also outperforms MMGM in clustering accuracy (cf. Table
\ref{tab:NUS_ImageClustering-1}) and computationally more efficient.
MMGM \cite{Chen_2014Robust} requires heavier computation than our
models due to its max-margin multiclass formulation that uses the
Reused Algorithm to jointly estimate two variables: the best and
the second best label assignments. The complexity is hence roughly
quadratic in the number of current clusters $\mathcal{O}\left(K^{2}\right)$,
while sampling $z_{i}$ in our model only takes $\mathcal{O}(K)$.
 
\begin{figure}
\centering{}\includegraphics[width=0.96\columnwidth]{figs/supplement/Clustering_wrt_Sigma_simplified}\caption{NUS Wide: model behavior w.r.t. $\Sigma_{0}=w\times\protect\idenmat$.
As $w$ increases from $\left[10^{-6},10^{1}\right]$, the norm of
$\eta$ is likely to increase making the model more discriminative
and reduce the number of cluster $K$ from $19$ to $17$.\label{fig:Model-behavior-Sigma_0}}
\end{figure}


\subsubsection{Model analysis}

\begin{table*}
\begin{centering}
\begin{tabular}{|l|c|c|c||c|c|c|c|c|c|}
\hline 
\multicolumn{3}{|c|}{Datasets} & \multirow{2}{*}{Metric} & \multicolumn{3}{c|}{Non-sequential} & \multicolumn{3}{c|}{Sequential}\tabularnewline
\cline{1-3} \cline{5-10} 
User & N & D &  & DPM & DDPM-S & DDPM-L & IHMM & DIH-S & DIH-L\tabularnewline
\hline 
\hline 
\multirow{2}{*}{A} & \multirow{2}{*}{3932} & \multirow{2}{*}{1114} & NMI & .275(.01) & .253(.008) & .246(.026) & \textbf{.305(.028)} & .254(.035) & \textbf{\emph{.276(.010)}}\tabularnewline
\cline{4-4} 
 &  &  & F1 & .473(.03) & \textbf{.526(.009)} & .466(.024) & .441(.018) & .480(.047) & \textbf{\emph{.483(.004)}}\tabularnewline
\cline{1-4} 
\noalign{\vskip-10pt}
 &  &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \tabularnewline
\hline 
\multirow{2}{*}{B} & \multirow{2}{*}{1793} & \multirow{2}{*}{185} & NMI & .245(.006) & .253(.006) & .253(.003) & .235(.023) & \textbf{\emph{.254(.002)}} & \textbf{.257(.003)}\tabularnewline
\cline{4-4} 
 &  &  & F1 & .535(.007) & \textbf{\emph{.553(.006)}} & .551(.001) & .481(.071) & \textbf{.559(.007)} & .543(.003)\tabularnewline
\cline{1-4} 
\noalign{\vskip-10pt}
 &  &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \tabularnewline
\hline 
\multirow{2}{*}{C} & \multirow{2}{*}{6623} & \multirow{2}{*}{1095} & NMI & .199(.01) & .216(.023) & .208(.014) & \textbf{\emph{.221(.021)}} & \textbf{.222(.006)} & .219(.004)\tabularnewline
\cline{4-4} 
 &  &  & F1 & \textbf{\emph{.672(.01)}} & .657(.010) & .641(.031) & .645(.003) & .659(.008) & \textbf{.673(.034)}\tabularnewline
\hline 
\end{tabular}
\par\end{centering}
\begin{centering}
\par\end{centering}
\caption{Clustering evaluation on time-series data using non-sequential and
sequential methods.\label{tab:Clustering-performance-evaluatio_timeseries}}
\end{table*}
We study the sensitivity of our discriminative model through the parameter
$\Sigma_{0}$ which plays an interesting role in controlling our
model discriminative property. Let $\Sigma_{0}=w\times\idenmat$ for
$w>0$. As $w\rightarrow0$ (cf. Eq. (\ref{eq:sampling_etak_dpm})),$\forall k$,
$\eeta_{k}$ approaches zero; hence there is no effect of discrimination,
and our model reduces to the standard generative model of DPM. As
$w$ increases, the norm of $\eta$ is also likely to increase, making
the discrimination effect stronger.

We vary the value of $w$ and measure performance on the NUS Wide
dataset. As can be seen from Fig. \ref{fig:Model-behavior-Sigma_0},
the NMI score increases as soon as a small discriminative factor is
introduced ($w=10^{-6}$). In terms of the number of clusters, when
we force our model to be more discriminative, our DDPM tends to get
less clusters, reducing $K$ from $19$ to $17$. We also notice the
\emph{robustness} of our model in the choice of $\Sigma_{0}$. For
a wide range of $w\in\left[10^{-6},10^{1}\right]$, our model consistently
obtains better performance than the DPM.

\subsection{DIH for Time-Series Analysis}

We evaluate the proposed discriminative-state iHMM using sequential
data on location dynamic discovery from the MDC dataset \cite{Laurila_12Mobile}.
We pick three users, denoted as A, B and C. Each user has the WiFi
access points recorded overtime using a smart phone.

We aim to discover the sequence of routine locations of each user.
Each inferred location is represented in our model a state or a cluster
of WiFi usage patterns. The clustering performance is then measured
using the ground truth provided. We compare discriminative-state
iHMM (DIH-S and DIH-L) with the iHMM, as well as models for i.i.d.
data (DDPM and DPM). Our main competitor is the iHMM \cite{Beal_etal_02infinite}
which utilizes the Markov property to exploit the sequential dependency
and can identify the suitable number of clusters for time series data.

The clustering performance is reported in Table \ref{tab:Clustering-performance-evaluatio_timeseries}.
The results show that our discriminative-state iHMMs consistently
outperforms the standard iHMM. The DIH-S performs slightly better
than DIH-L, and is generally the best method against all the baselines.
\begin{figure}
\begin{centering}
\includegraphics[width=1\columnwidth]{figs/experiment_timeseries/Clustering_Performance_wrt_Time}
\par\end{centering}
\caption{The performance w.r.t. CPU time on User A. \label{fig:Clustering-analysis_wrt_Time}}
\end{figure}

We further illustrate the advantage of our discriminative models by
visualizing how the clustering performance (F1-score) improves as
a function of CPU times in Fig. \ref{fig:Clustering-analysis_wrt_Time}.
Since our method might take longer time in each Gibbs iteration
comparing to the iHMM, to have a fair comparison, we take the time
spent per iteration into the assessment. We observe that our discriminative
iHMM take less time to achieve a sufficiently good and stable clustering
result. Although not definitive, this behavior suggests that the augmented
Gibbs sampler developed for our discriminative iHMM is mixing just
as well as the collapsed Gibbs sampler on iHMM, if not faster.



